REORDER: Securing Dynamic-Priority Real-Time Systems Using Schedule Obfuscation

The deterministic (timing) behavior of real-time systems (RTS) can be used by adversaries - say, to launch side channel attacks or even destabilize the system by denying access to critical resources. We propose a protocol (named REORDER) to obfuscate this predictable timing behavior of RTS, especially ones designed using dynamic-priority scheduling algorithms (e.g., EDF). We also present a metric (named "schedule entropy") that measures the levels of obfuscation introduced into a given real-time system. The REORDER protocol was integrated into the standard Linux real-time scheduler and evaluated on a realistic embedded platform (Raspberry Pi) running the MiBench automotive benchmark workloads. We also demonstrate how designers of RTS can increase the security of their systems and also quantitatively measure the impact (both in terms of security and performance) of using this protocol.

==> Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

LATEX = pdflatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> Sections/eval_synthetic.tex <==
In this section, we evaluate \papername using a prototype implemented on an embedded platform (\ie RPi3) running the real-time Linux kernel (Section \ref{subsec:linux}). The key observations from our performance evaluation results are summarized below.
\todo[inline]{Sibin: Move the following first two points to section IV.}
\begin{itemize}
\item The randomization protocol works best when the system has low to medium load. Also for higher utilizations the benefits of idle time scheduling is not significant compared to the base randomization scheme (Fig. \ref{fig:entropy}). 

\item Compared to vanilla EDF, randomization allows tasks to appear in wider ranges (specially for higher utilizations) that would make it hard for the attackers to infer actual task execution time (Fig. \ref{fig:wcrt-ratio}).

\item \papername \hl{works in practice on realistic embedded RTS and is able to meet the real-time guarantees.}

\item The randomization logic adds minimal scheduling overhead in Linux kernel (Fig. \ref{fig:pick_next_task_cost}).
This overhead is arguably very small in comparison with the task execution time (Fig. \ref{fig:cost_ratio}).
%Our prototype on Linux shows that \papername is more likely to select a random task when the system has more tasks (Fig. \ref{fig:random_task_proportion}).
\end{itemize}


==> Sections/th_proof.tex <==
\subsection{Proof of Theorem \ref{th:ibf}} \label{appsec:ibf_proof}

% \begin{IEEEproof}
We prove the assertion following an approach similar to that of prior work \cite{Baker_SSR, priority_inversion_sanjay}. Let us assume that some deadlines are missed due to priority inversion. Let $t_\phi$ be the first time a job misses its deadline and $t_\phi^\prime$ be the last time (before $t_\phi$) when there are no pending job execution requests with arrival times before $t_\phi^\prime$ and deadlines before or at $t_\phi$. For instance, let us consider that $\tau_i$ is blocked by some low priority task $\tau_j$. Note that there could be at most one job (with deadline $>t_\phi$) that executes in the interval $[t_\phi^\prime, t_\phi)$ \cite{Baker_SSR}, hence the following condition will hold: $d_i \leq t_\phi^\prime - t_\phi$ -- since no job with deadline $>t_\phi$ could possibly become blocked during the interval $[t_\phi^\prime, t_\phi)$. Therefore  at most $\mathsf{IBF}(t_\phi - t_\phi^\prime)$ of the execution over $[t_\phi^\prime, t_\phi)$ can be of a low priority task $\tau_j$ with $d_j > t_\phi$. Since a deadline is missed at time $t_\phi$, the cumulative demand $\mathsf{IBF}(t_\phi - t_\phi^\prime) + \sum\limits_{\tau_i \in \Gamma} \mathsf{DFB}(\tau_i, t_\phi - t_\phi^\prime)$ must exceed the length of the interval. Letting $t \overset{\operatorname{def}}{=} t_\phi - t_\phi^\prime$, the following condition  must hold to  ensure that no deadline will be missed:
\begin{equation}
\mathsf{IBF}(t) + \sum\limits_{\tau_i \in \Gamma} \mathsf{DFB}(\tau_i, t) \leq t, ~\forall t \geq 0.
\end{equation}
Rearranging the terms in above equation we obtain the following: $\mathsf{IBF}(t) \leq t -   \sum\limits_{\tau_i \in \Gamma} \mathsf{DFB}(\tau_i, t), ~\forall t \geq 0$. Therefore the priority inversion budget is upper bounded by Eq. (\ref{eq:ibf_proof})
and the proof follows. 
% \end{IEEEproof}
